Language Models of Code are Few-Shot Commonsense Learners

We address the general task of structured commonsense reasoning: given a natural language input, the goal is to generate a graph such as an event -- or a reasoning-graph. To employ large language models (LMs) for this task, existing approaches ``serialize'' the output graph as a flat list of nodes and edges. Although feasible, these serialized graphs strongly deviate from the natural language corpora that LMs were pre-trained on, hindering LMs from generating them correctly. In this paper, we show that when we instead frame structured commonsense reasoning tasks as code generation tasks, pre-trained LMs of code are better structured commonsense reasoners than LMs of natural language, even when the downstream task does not involve source code at all. We demonstrate our approach across three diverse structured commonsense reasoning tasks. In all these natural language tasks, we show that using our approach, a code generation LM (CODEX) outperforms natural-LMs that are fine-tuned on the target task (e.g., T5) and other strong LMs such as GPT-3 in the few-shot setting.

==> figures/proscript_example_tree.tex <==
\begin{tikzpicture}[node distance=0.9cm]
\newcommand{\nodespacing}{3pt}
\newcommand{\roundness}{2mm}
\newcommand{\proparamarkersize}{1.5mm}
% \footnotesize % pun unintended
    \node [rectangle,draw=white,fill=gray!20,] (title) {Scenario: \emph{bake a cake}};
    \node [draw, right of=title, xshift=3cm, yshift=-3mm, rounded corners=\roundness,inner sep=2pt] (node0) {find the cake recipe};
    \node [draw, below of=node0, xshift=-2.5cm, rounded corners=\roundness,inner sep=\nodespacing]  (node1) {gather the ingredients};
    \node [draw, below of=node0, xshift=0.5cm, yshift=-0.5cm, rounded corners=\roundness,inner sep=\nodespacing] (node2) {turn on the oven};
    \node [draw, below of=node1, rounded corners=\roundness,inner sep=\nodespacing] (node3) {mix the ingredients};
    \node [draw, below of=node3, xshift=1.5cm,rounded corners=\roundness,inner sep=\nodespacing] (node4) {put the cake batter in the oven};
    \node [draw, below of=node4, rounded corners=\roundness,inner sep=\nodespacing] (node5) {bake for the right amount of time};
    \node [draw, below of=node5, rounded corners=\roundness,inner sep=\nodespacing] (node6) {take the cake out of the oven};
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node0) -- (node1);
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node0) -- (node2);
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node1) -- (node3);
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node3) -- (node4);
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node2) -- (node4);
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node4) -- (node5);
    \draw [-{Latex[length=\proparamarkersize, line width=1pt]}] (node5) -- (node6);
\end{tikzpicture}

==> scratchpad/intro.tex <==
\section{Introduction}
The key ideas \corr{is}{are} this:
\begin{enumerate}
    \item \hlite{Structured commonsense generation}
    \item \hlite{How are these models typically trained?}
    \item \hlite{What are the shortcomings of these models}
    \item \hlite{Code generation models can help}
    \item \hlite{Our main research question}
    \item \hlite{Contributions} 
\end{enumerate}

\aman{Add citations everywhere}

\hlite{Structured commonsense generation}

The\uri{\sout{se}} growing capabilities of \uri{large} pre-trained language models \uri{"(LLMs)", so we can use this term later} for generating text have enabled their successful application on a diverse set of tasks, including summarization, translation, question-answering, \uri{"and also in ", to emphasize the distinction between NL-LMs and Code-LMs} code \cite{chen2021evaluating,austin2021program,xu2022systematic}, and graph generation \uri{ I would remove "graph generation", because it's not as obvious and well known as the other applications}.
Subsequently, there is now a growing interest in tackling traditionally discriminative tasks in a generation setup. \uri{This is more of a technical detail that I'm not sure that is required this early}
A popular example of this shift appears in commonsense reasoning, where structured commonsense generation is getting increasingly popular.
Unlike traditional commonsense reasoning tasks involving reading comprehension or question answering, structured commonsense generation aims to extract structures from the given input.
Some examples of structured commonsense tasks include generating event graphs, reasoning graphs, scripts given a goal, and argument explanation graphs.

\uri{Suggesting a rephrase, starting from "Subsequently": 
Nevertheless, while applying LLMs for these tasks is straightforward, a major remaining challenge is how to leverage LLMs in \emph{structured commonsense reasoning}. 
Unlike traditional commonsense reasoning tasks such as reading comprehension or question answering, structured commonsense aims to extract \emph{structures} from a given input.
This task requires the natural language knowledge learned by the LLM,
but it also requires complex structured prediction and generation.
Some examples of structured commonsense tasks include generating event graphs, reasoning graphs, scripts, and argument explanation graphs. 
}

\hlite{How are these models typically trained? } Typically, structured commonsense generation models adapt the problem setup ("setup" is a little too vague, how about "format"?) to leverage LLMs.
Specifically, the structure to be generated~(\eg a graph or a table) is converted, or ``serialized'', to text.
Common ways to achieve this include flattening the graph into a list of tuples, or serializing graphs into specification language such as \dotf. 
These transformations reduce the problem to text-to-text generation and allow direct use of language models.

\hlite{What are the issues?} While this approach of converting the structured output to text is convenient and has shown promising results, the encoding does not capture the semantics of the input \uri{the last part bothers me, because the encoding *does* capture the semantics of the input in the sense that the encoding can be "decoded" back to its previous form. How about first presenting the second argument, which is more straightforward:}.
Further, language models are typically pre-trained on free-form text, and thus are not explicitly trained for structured prediction.
\uri{and then go back to the first argument, which is a little more subtle: "Further, to perfectly encode the semantics of the original inputs, the transformation into a serialized graph makes it more difficult to directly express and learn the semantics."}
Consequently, these systems typically require an extensive \uri{a large?} training set, and the generated output shows semantic and structural issues, that either need manual fixes or secondary training~\citep{madaan2021think}.

\uri{Suggesting a rephrase for the entire previous paragraph:}
While this approach of converting the structured output to text has a  deterministic, closed-form, formula and it has shown promising results \cite{cite,cite,cite}, LLMs struggle to learn to generate these  ``unnatural'' outputs: 
language models are typically pre-trained on free-form text, 
and these serialized structured outputs strongly diverge from the model's pre-training data. 
Further, 
%to perfectly encode the semantics of the original graphs, 
the transformation into a serialized graph pushes dependent pieces of text farther apart, which
makes it difficult for the model to directly learn the relation between them.
Consequently, these models typically require large training sets and their generated outputs show structural errors and semantic inconsistencies. These errors and inconsistencies later need to be fixed either manually or using a secondary downstream model~\citep{madaan2021think}.
\uri{A good figure would go a long way here: example of an input, the graph output, a bad but straightforward encoding, and "our approach" of encoding?}

\hlite{Code generation models can overcome some of these challenges} 
Despite these struggles, the recent success of large-language models of \emph{code} \cite{chen2021evaluating,austin2021program,wang2021codet5,xu2022systematic,fried2022incoder} show that \uri{\sout{the formulation of structured commonsense generation as a text-to-text problem is indeed promising.}}
LLMs of code \emph{are able} to perform complex reasoning in structured text, \emph{if pre-trained on the right data}.
\uri{\sout{A key difference in the two setups is the availability of a large pre-training corpus:  while structured commonsense generation models are fine-tuned on relatively small training data for isolated tasks, code generation models leverage a large open-source corpus of code for pre-training. Combined with a large model architecture, code generation models trained in this fashion learn to generate code in various languages and show impressive results on challenging tasks like text-to-code generation.}}
\uri{Rephrashing:}
In other words, instead of forcing LLMs of natural language to be fine-tuned on structured commonsense data, an easier way to close the gap between the pre-training data (free-form text) and the task-specific data (commonsense reasoning) would be to \emph{adapt LLMs that were pre-trained on code to structured commonsense reasoning}.


\hlite{Our main research question} In this work, \uri{\sout{we explore the possibility of utilizing code generation models for structured commonsense generation, and}} we show how large language models of \emph{code} can be useful for \emph{natural language} commonsense reasoning. Further, we show that LLMs of code can be even better reasoners than LLMs of natural language.
We make the following contributions: 
\begin{compactenum}
    \item We propose \ours{} \uri{(\textsc{cocogen} or \textsc{CoCoGen}?)}: a method for leveraging LLMs of \textbf{co}de for structured \textbf{co}mmonsense \textbf{gen}eration.
    \item We outline novel methods of dynamically curating the in-context examples for \ours \uri{- unclear (I don't even know what it means?)}
    \item We perform exhaustive analysis and human evaluation \uri{human evaluation???}, highlighting the key strengths and shortcomings of \ours. \uri{consider removing this item}
    \item We perform thorough evaluation across three diverse structured commonsense generation tasks, showing that \ours{} vastly outperforms natural language LLMs, either fine-tuned or few-shot tested, while controlling for the number of task-specific examples, and is competitive with models fine-tuned with orders of magnitude more data.
    \item We perform an extensive ablation study, which show the role of data formatting, model size, and the number of few-shot examples.
\end{compactenum}
% i) we provide \ours, a method for using code-generation models for structured commonsense generation in a few-shot setup; ii) our experiments on three diverse structured commonsense generation tasks show that \ours vastly outperforms fine-tuned models controlling for the available data, and is competitive with models fine-tuned with orders of magnitude more data; iii) we outline novel methods of dynamically curating the in-context examples for \ours, and iv) we perform exhaustive analysis and human evaluation, highlighting the key strengths and shortcomings of \ours. Our ablation analysis also reveals the role of format, model size, and the number of examples.


==> sections/abstract_plain_text.tex <==
We address the general task of structured commonsense reasoning: given a natural language input, the goal is to generate a graph such as an event or a reasoning-graph.
To employ large language models (LMs) for this task, existing approaches 'serialize' the output graph as a flat list of nodes and edges.
Although feasible, these serialized graphs strongly deviate from the natural language corpora that LMs were pre-trained on, hindering LMs from generating them correctly. 
In this paper, we show that when we instead frame structured commonsense reasoning tasks as code generation tasks, pre-trained LMs of code are better structured commonsense reasoners than LMs of natural language, even when the downstream task does not involve source code at all.
We demonstrate our approach across three diverse structured commonsense reasoning tasks. In all these natural language tasks, we show that using our approach, a code generation LM~(codex) outperforms natural-LMs that are fine-tuned on the target task (T5) and other strong LMs such as GPT-3 in the few-shot setting.
